Energy Reduction Opportunities in HDR Video Encoding

This paper investigates the energy consumption of video encoding for high dynamic range videos. Specifically, we compare the energy consumption of the compression process using 10-bit input sequences, a tone-mapped 8-bit input sequence at 10-bit internal bit depth, and encoding an 8-bit input sequence using an encoder with an internal bit depth of 8 bit. We find that linear scaling of the luminance and chrominance values leads to degradations of the visual quality, but that significant encoding complexity and thus encoding energy can be saved. An important reason for this is the availability of vector instructions, which are not available for the 10-bit encoder. Furthermore, we find that at sufficiently low target bitrates, the compression efficiency at an internal bit depth of 8 bit exceeds the compression efficiency of regular 10-bit encoding.

==> gfx/RCD_energy_vid4_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{017}[tc][tc]{ Relative Rate Difference (%)}%
\psfrag{018}[bc][bc]{ PSNR}%
\psfrag{019}[tc][tc]{ Rate}%
\psfrag{020}[bc][bc]{ PSNR}%
\psfrag{000}[ct][ct]{ $- 20$}%
\psfrag{001}[ct][ct]{ $- 10$}%
\psfrag{002}[ct][ct]{ $0$}%
\psfrag{003}[ct][ct]{ $10$}%
\psfrag{004}[ct][ct]{ $20$}%
\psfrag{005}[ct][ct]{ $30$}%
\psfrag{006}[ct][ct]{ $40$}%
\psfrag{011}[ct][ct]{ 10^{3}}%
\psfrag{012}[ct][ct]{ 10^{4}}%
\psfrag{007}[rc][rc]{ $8$}%
\psfrag{008}[rc][rc]{ $8.5$}%
\psfrag{009}[rc][rc]{ $9$}%
\psfrag{010}[rc][rc]{ $9.5$}%
\psfrag{013}[rc][rc]{ $8$}%
\psfrag{014}[rc][rc]{ $8.5$}%
\psfrag{015}[rc][rc]{ $9$}%
\psfrag{016}[rc][rc]{ $9.5$}%
%
%% </ytick>

==> gfx/rd_RCD_v4_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{015}[tc][tc]{ Relative Rate Difference (%)}%
\psfrag{016}[bc][bc]{ PSNR}%
\psfrag{017}[tc][tc]{ Rate}%
\psfrag{018}[bc][bc]{ PSNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
\psfrag{000}[ct][ct]{ $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{ $0$}%
\psfrag{002}[ct][ct]{ $100$}%
\psfrag{003}[ct][ct]{ $200$}%
\psfrag{004}[ct][ct]{ $300$}%
\psfrag{005}[ct][ct]{ $400$}%
\psfrag{006}[ct][ct]{ $500$}%
\psfrag{007}[ct][ct]{ $600$}%
\psfrag{011}[ct][ct]{ 10^{0}}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{ $40$}%
\psfrag{009}[rc][rc]{ $45$}%
\psfrag{010}[rc][rc]{ $50$}%
\psfrag{012}[rc][rc]{ $40$}%
\psfrag{013}[rc][rc]{ $45$}%
\psfrag{014}[rc][rc]{ $50$}%
%
%% </ytick>

==> gfx/rvdp_RCD_v4_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{015}[tc][tc]{ Relative Rate Difference (%)}%
\psfrag{016}[bc][bc]{ PSNR}%
\psfrag{017}[tc][tc]{ Rate}%
\psfrag{018}[bc][bc]{ PSNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
\psfrag{000}[ct][ct]{ $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{ $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{ $0$}%
\psfrag{003}[ct][ct]{ $20$}%
\psfrag{004}[ct][ct]{ $40$}%
\psfrag{005}[ct][ct]{ $60$}%
\psfrag{010}[ct][ct]{ 10^{0}}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{ $8$}%
\psfrag{007}[rc][rc]{ $8.5$}%
\psfrag{008}[rc][rc]{ $9$}%
\psfrag{009}[rc][rc]{ $9.5$}%
\psfrag{011}[rc][rc]{ $8$}%
\psfrag{012}[rc][rc]{ $8.5$}%
\psfrag{013}[rc][rc]{ $9$}%
\psfrag{014}[rc][rc]{ $9.5$}%
%
%% </ytick>

==> gfx/vdp_encTime_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{010}[tc][tc]{ Rate}%
\psfrag{011}[bc][bc]{ PSNR}%
\psfrag{000}[ct][ct]{ $0$}%
\psfrag{001}[ct][ct]{ $200$}%
\psfrag{002}[ct][ct]{ $400$}%
\psfrag{003}[ct][ct]{ $600$}%
\psfrag{004}[ct][ct]{ $800$}%
\psfrag{005}[rc][rc]{ $8$}%
\psfrag{006}[rc][rc]{ $8.5$}%
\psfrag{007}[rc][rc]{ $9$}%
\psfrag{008}[rc][rc]{ $9.5$}%
\psfrag{009}[rc][rc]{ $10$}%
%
%% </ytick>

==> gfx/vdp_energy_v1_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
\psfrag{009}[tc][tc]{ Rate}%
\psfrag{010}[bc][bc]{ PSNR}%
\psfrag{000}[tc][tc]{ $\times10^{4}$}%
\psfrag{001}[ct][ct]{ $0$}%
\psfrag{002}[ct][ct]{ $0.5$}%
\psfrag{003}[ct][ct]{ $1$}%
\psfrag{004}[ct][ct]{ $1.5$}%
\psfrag{005}[ct][ct]{ $2$}%
\psfrag{006}[rc][rc]{ $8$}%
\psfrag{007}[rc][rc]{ $9$}%
\psfrag{008}[rc][rc]{ $10$}%
%
%% </ytick>
